"Is your explanation stable?": A Robustness Evaluation Framework for Feature Attribution

Understanding the decision process of neural networks is hard. One vital method for explanation is to attribute its decision to pivotal features. Although many algorithms are proposed, most of them solely improve the faithfulness to the model. However, the real environment contains many random noises, which may leads to great fluctuations in the explanations. More seriously, recent works show that explanation algorithms are vulnerable to adversarial attacks. All of these make the explanation hard to trust in real scenarios. To bridge this gap, we propose a model-agnostic method \emph{Median Test for Feature Attribution} (MeTFA) to quantify the uncertainty and increase the stability of explanation algorithms with theoretical guarantees. MeTFA has the following two functions: (1) examine whether one feature is significantly important or unimportant and generate a MeTFA-significant map to visualize the results; (2) compute the confidence interval of a feature attribution score and generate a MeTFA-smoothed map to increase the stability of the explanation. Experiments show that MeTFA improves the visual quality of explanations and significantly reduces the instability while maintaining the faithfulness. To quantitatively evaluate the faithfulness of an explanation under different noise settings, we further propose several robust faithfulness metrics. Experiment results show that the MeTFA-smoothed explanation can significantly increase the robust faithfulness. In addition, we use two scenarios to show MeTFA's potential in the applications. First, when applied to the SOTA explanation method to locate context bias for semantic segmentation models, MeTFA-significant explanations use far smaller regions to maintain 99\%+ faithfulness. Second, when tested with different explanation-oriented attacks, MeTFA can help defend vanilla, as well as adaptive, adversarial attacks against explanations.

==> sections/significance_test_old.tex <==
\section{Significance Test}
First, in \ref{3.1} we introduce the notation of this paper. Then, In \ref{3.2} we demonstrate the first part of ST, which allows to give a significant salient region according to a given salient value threshold. Next, in \ref{3.3} we introduce the second part of ST, which allows to give the confidence interval with $\alpha$ confidence of every pixel and output the overall confidence of this explanation.

\subsection{Preliminary}\label{3.1}
Let $f:\ \mathbb{R}^{c\times w\times h}\rightarrow\mathbb{R}^C$ be a predict function, which maps an image to the confidence vector, where $c$, $w$, $h$ are the respective the number of channels, width and height of the input, and $C$ is the number of the classes. Let $F$ be the set of prediction functions satisfying the above definition. $ve$ is a visual explanation method, mapping a predict function and an image to a saliency map M. Formally, $ve: F\times\mathbb{R}^{c\times w\times h}\rightarrow[0,1]^{w\times h}$. 

However, as we said above, the saliency map obtained is probably unstable and inaccurate\TBD{Add Reference}. Thus, our method(ST) builds on top of SmoothGrad\TBD{Add Reference}, in which authors try to drop out noisy values in saliency map by adding small noise to the original image and averaging all of the saliency maps. ST gets a saliency map by add noise, which just slightly changes the predict vector of $f$. Formally, $M=ve(f,I+n)$, where I is the original image, $n\sim \mathcal{N}$ is noise of dimension $w\times h$. Let $\mathcal{M}$ denote the distribution of $M$. For a saliency value $v$ of interest, let $ct(v,p,N)=\sum_{i=0}^{N-1}I(M(p)\geq v)$, where $I(\cdot )$ is indicator function, $N$ is the number of samples, and $M(p)$ is the saliency value of pixel $p$ in $M$.
% The definition of median is only for the continuous random variable. However, There exists a kind of visual explanation method output discrete saliency value(e.g. LIME). So we extend the definition of median as follows:
% \begin{definition}
% A number $m\in \mathbf{R}$ is the median of a random variable $X$, if for any number $x<m$, $P(X\leq x)<0.5$ and $P(X\leq m)\geq 0.5$.
% \end{definition}
\subsection{Our Goal}
As we said before, the explanation methods give a distribution $\mathcal{M}$. However, we could not give a distribution to user to explain the prediction of the model. In fact, we need to select a most representative saliency map to explain the prediction of the model. In this paper, we select the center of the distribution, i.e. the median, as the most representative saliency map. However, the definition of median is only for the continuous random variable and sometimes not unique. Thus we extend the definition of median as follows:
\begin{definition}
A number $m\in \mathbf{R}$ is the median of a random variable $X$, if for any number $x<m$, $P(X\leq x)<0.5$ and $P(X\leq m)\geq 0.5$.
\end{definition}
Although it is impossible to sample a distribution a limited number of times to determine the median, we can make some estimates of its properties. In \ref{3.2}, we design one-sided test to find out if the median is really greater than a threshold of interest. Further, in \ref{3.3}, we design two-sided test to give the confidence interval of the median of any pixel. Finally, the overall confidence of the explanation is given according to the length of the confidence interval.

\subsection{One-sided test}\label{3.2}

In one-sided test, ST aims to find out that one pixel with high saliency value, or specifically, saliency value greater than a margin $v$ is a real property? ST samples $N$ saliency maps $M\sim\mathcal{M}$ and designs a one-sided test as follows:

\begin{theorem}\label{hard-margin}

\begin{itemize}
    \item If $ct(v,p,N)\leq k_1$, where $k_1 = \max\{k|C_N^k\cdot prob^k\cdot (1-prob)^{N-k}<\alpha,\ k=0,1,...,N-1\},\ prob = \min\{0.5,k/N\}$, then under the confidence $\alpha$, the median of $M(p)$ is smaller than $v$.
    \item If $ct(v,p.N)\geq k_2$, where $k_2 = \min\{k|C_N^k\cdot prob^k\cdot (1-prob)^{N-k}<\alpha,\ k=0,1,...,N-1\},\ prob = \min\{0.5,k/N\}$, then under the confidence $\alpha$, the median of $M(p)$ is greater than $v$.
\end{itemize}

\end{theorem}

ST thus calculates the statistical significance of each pixel using \ref{hard-margin}, and outputs a three-value map named significance map $S$ according to significantly greater than v, significantly less than v, and insignificant. 
The specific implementation steps are detailed in \ref{algorithm1}

\begin{algorithm}[tb]
\caption{One-sided test}
\label{algorithm1}
\textbf{Input}: visual explanation method $ve$, image $I$, predict function $f$, target saliency value $v$\\
\textbf{Parameter}:confidence $\alpha$, number of saliency maps $N$\\
\textbf{Output}: significance map $S$
\begin{algorithmic}[1] %[1] enables line numbers
\STATE Let $t=0$.
\FOR{i = 0:N-1}
\STATE sample noise $n$ from $\mathcal{N}$
\STATE record map $M_i = ve(f,I+n)$)
\ENDFOR
\STATE compute $k_1$ and $k_2$ according to \ref{hard-margin}
\STATE create an empty matrix $S\in\mathbf{R}^{w\times h}$
\FOR{every pixel p in S}
\IF{$ct(p,v,N)\geq k_2$}
\STATE $S(p)=1$
\ELSIF{$ct(p,v,N)\leq k_1$}
\STATE $S(p)=-1$
\ELSE
\STATE $S(p)=0$
\ENDIF
\ENDFOR
\STATE \textbf{return} $S$
\end{algorithmic}
\end{algorithm}

%\begin{algorithm}
%\caption{One-sided test}\label{algorithm1}
%\SetAlgoLined
%\SetKwInOut{Parameter}{Parameter}
%\KwIn{visual explanation method $ve$, image $I$, predict function $f$, target saliency value $v$}
%\Parameter{confidence $\alpha$, number of saliency maps $N$}
%\KwOut{significance map $S$}
%\For{i = 0:N-1}{
%    sample noise $n$ from $\mathcal{N}$\\
%    record map $M_i = ve(f,I+n)$)
%}
%compute $k_1$ and $k_2$ according to \ref{hard-margin}\\
%create an empty matrix $S\in\mathbf{R}^{w\times h}$\\
%\For{every pixel p in S}{
%  \uIf{$ct(p,v,N)\geq k_2$}{
%    $S(p)=1$ \\
%  }
%  \uElseIf{$ct(p,v,N)\leq k_1$}{
%    $S(p)=-1$ \\
%  }
%  \Else{
%    $S(p)=0$ \\
%  }
%
%}
%return $S$
%\end{algorithm}



\subsection{Two-side test}\label{3.3}
% One of the advantages of saliency map is that its value is the continuous interval of [0,1]. Compared with discrete values, such as {0,1}, the saliency map can compare the contribution of any two pixels. In order to preserve such property, we design a two-side test to find the confidence interval of the median of $M(p)$

Further, we want to know how large is the change interval of the saliency value of the pixels? Saliency value of one pixel is an random variable, so we can estimate its median. By counting $N$ saliency values, ST can construct a two-sided test to give the confidence interval of the median of any pixel.

\begin{theorem}\label{confidence interval}

Supposing $N$ number $x_0\leq x_1\leq...\leq x_{N-1}$ are the saliency value of pixel $p$, letting $k_1 = \arg\max\{k:\sum_{i=0}^{k}\cdot0.5^N\cdot C_N^{k}\leq \alpha/2\}$, $k_2 = N-k_1$, then $[x_{k_1},x_{k_2-2}]$ is a $(1-\alpha)$ confidence interval of the median of $M(p)$

\end{theorem}

The length of the confidence interval can reflect the variation of the variable. The longer the confidence interval, the greater the variation of the variable, and the less credible; the shorter the confidence interval, the smaller the variation of the variable, the more credible it is. Thus we define the overall confidence of one saliency map as follows:

\begin{definition}\label{overall confidence}
Let $[lb(p),hb(p)]$ denote the $\alpha$ confidence interval of the median of $M(p)$. Then overall confidence $oc := 1-\frac{\sum_p(hb(p)-lb(p))}{\sum_p 1}$
\end{definition}

Since the saliency value is in $[0,1]$, thus $oc$ is in $[0,1]$. It's easy to find out that the higher the $oc$, the shorter the average confidence interval length, and the more credible. The specific implementation steps are detailed in \ref{algorithm2}

\begin{algorithm}[tb]
\caption{Two-sided test}
\label{algorithm2}
\textbf{Input}: visual explanation method $ve$, image $I$, predict function $f$\\
\textbf{Parameter}:confidence $\alpha$, number of saliency maps $N$\\
\textbf{Output}: lower bound map $LB$, higher bound map $HB$, overall confindence $oc$
\begin{algorithmic}[1] %[1] enables line numbers
\STATE Let $t=0$.
\FOR{i = 0:N-1}
\STATE sample noise $n$ from $\mathcal{N}$
\STATE record map $M_i = ve(f,I+n)$)
\ENDFOR
\STATE compute the $k_1,\ k_2$ according to \ref{confidence interval}
\STATE stack $M_i$ and sort them in the new channel
\STATE slice the map $k_1$ and map $k_2-2$ in sorted maps as $LB$ and $HB$
\STATE compute $oc$ with $LB$ and $HB$ according to \ref{overall confidence}
\STATE \textbf{return} $S$
\end{algorithmic}
\end{algorithm}

%\begin{algorithm}
%\caption{Two-sided test}\label{algorithm2}
%\SetAlgoLined
%\SetKwInOut{Parameter}{Parameter}
%\KwIn{visual explanation method $ve$, image $I$, predict function $f$}
%\Parameter{confidence $\alpha$, number of saliency maps $N$}
%\KwOut{lower bound map $LB$, higher bound map $HB$, overall confindence $oc$}
%\For{i = 0:N-1}{
%    sample noise $n$ from $\mathcal{N}$\\
%    record map $M_i = ve(f,I+n)$)
%}
%compute the $k_1,\ k_2$ according to \ref{confidence interval}\\
%stack $M_i$ and sort them in the new channel\\
%slice the map $k_1$ and map $k_2-2$ in sorted maps as $LB$ and $HB$\\
%compute $oc$ with $LB$ and $HB$ according to \ref{overall confidence}\\
%return $S$
%\end{algorithm}


